Learning Fractional-Order Dynamics from a Single Trajectory

Many real-world processes exhibit long-range dependence, where the current state depends on a slowly decaying trace of past states rather than on the most recent state alone. This paper studies system identification for discrete-time fractional-order linear time-invariant systems from a single observed trajectory of length $t$, a setting that captures such non-Markovian dynamics through the Gr\"unwald--Letnikov difference operator. Unlike Markovian systems, fractional-order systems couple estimation across the entire history, making both statistical analysis and practical identification more challenging. We propose \emph{Fractional-Order Ordinary-Least-Squares Grid-Search (FO-GS)}, a simple two-stage estimator that exploits the diagonal structure of the fractional-difference operator to decouple the identification problem row-wise. Under the stability assumption, we establish high-probability, non-asymptotic error bounds for estimating both the fractional order and the system matrix in the heterogeneous setting, with both estimation errors scaling as \(\mathcal{O}(t^{-1/2})\). Through experiments, we show that \emph{FO-GS} outperforms existing baselines in recovering both the fractional order and the underlying system dynamics.

==> rebuttal.tex <==
\section{Rebuttal}


\input{fast_rate_revised_modified (2)}
%\input{fast_rate_rebuttal}
\subsection{Reviewer VqoX }
\textcolor{red}{Question 1: Can Assumption 2 be replaced by a lemma that derives the constant  from the model primitives? As written, both Theorem 1's identifiability and the separation condition depend on a quantity that cannot be checked for a concrete system. Since you already prove the matching curvature lower bound in Lemma 12, this seems within reach.}

Yes. We can use the following lemma to replace Assumption 2: Under Assumption 1, for each $i\in[n]$ and for every
$\alpha_i\in[\frac{\alpha_{i,\star}}{2},1]$,
\begin{align}
\frac1t\sum_{s=0}^{t-1}
\mathbb E\left|
 b_s^{(i)}(\alpha_i)
 -(\alpha_i-\alpha_{i,\star})
 \sum_{j\ge1}
 \partial_\alpha\psi(\alpha_{i,\star},j)
 x_{s+1-j}^{(i)}
\right|^2
\le
\frac{K_i^2}{4}
|\alpha_i-\alpha_{i,\star}|^4,
%\label{eq:taylor_remainder_explicit}
\end{align}
where $K_i = \frac{9e}{4}\sigma\tilde {C}_G\sqrt{\zeta(2)}
\bigl(\zeta\left(1+\frac{\alpha_{i,\star}}{2}\right)
-2\zeta'\left(1+\frac{\alpha_{i,\star}}{2}\right)
+\zeta''\left(1+\frac{\alpha_{i,\star}}{2}\right)\bigr).$
%$K_i = \frac{9e}{4} \sigma  \tilde{C}\_{G} \sqrt{\zeta(2)} (\zeta(1+\frac{\alpha_{i,\star}}{2}) - 2\zeta'(1+\frac{\alpha_{i,\star}}{2}) + \zeta''(1+\frac{\alpha_{i,\star}}{2}) )$

\textcolor{red}{Question 2: Is the $t^{-1/4}$ rate fundamental, or an artifact of grid search? A lower bound showing $t^{-1/4}$ is unavoidable would strengthen the paper; alternatively, improving the proof argument to achieve $t^{-1/2}$  would also be a strong improvement.}

Thank you for raising this important point. The $t^{-1/4}$ rate is not intrinsic to \textit{FO-GS}; it results from applying a $t^{-1/2}$ uniform-deviation bound to the squared loss and then taking a square root through local quadratic growth. We replace this step by a direct analysis of the unnormalized in-sample prediction error
$\mathcal E_t$. 
Define
\(
\mathcal Q_{t,i}(\alpha_i,a_i - a_{i,\star})
:=
\sum_{s=0}^{t-1}
\left|
\left(
\Delta^{\alpha_i}-\Delta^{\alpha_{i,\star}}
\right)x_{s+1}^{(i)}- \left(a_i - a_{i,\star}\right)x_s
\right|^2.
\)
%$\mathcal Q_{t,i}(\alpha_i,a_i - a_{i,\star}):=\sum_{s=0}^{t-1}\left|\left(\Delta^{\alpha_i}-\Delta^{\alpha_{i,\star}}\right)x_{s+1}^{(i)}- \left(a_i - a_{i,\star}\right)x_s\right|^2.$
The unnormalized in-sample prediction error $\mathcal E_t $ is
\[
\mathcal E_t
:=
\sum_{s=0}^{t-1}
\left\|
\left(
\Delta^{\widehat{\boldsymbol\alpha}}
-\Delta^{\boldsymbol\alpha_\star}
\right)x_{s+1}
-(\widehat A-A_\star)x_s
\right\|_2^2=
\sum_{i=1}^n
\mathcal Q_{t,i}
\left(
\widehat\alpha_i,
\widehat a_i-a_{i,\star}
\right).
\]
\iffalse
\\[
\mathcal E_t
:=
\sum_{s=0}^{t-1}
\lVert
(
\Delta^{\hat{\boldsymbol\alpha}}
-\Delta^{\boldsymbol\alpha_\star}
) x_{s+1}
-(\hat A-A_\star) x_s
\rVert_{2}^2 = \sum_{i=1}^n
\mathcal Q_{t,i}
(
\hat\alpha_i,
\hat a_i-a_{i,\star}
)
\\] 
\fi

Thus, $\mathcal Q_{t,i}$ is the contribution of row $i$, whereas
$\mathcal E_t$ is the sum over all rows. Martingale offset complexity
retains the negative quadratic term and yields
\[
\mathcal E_t
\le
c_1\theta t
\left\|
\widehat{\boldsymbol\alpha}
-\boldsymbol\alpha_\star
\right\|_\infty^2
+c_2t\epsilon_{\max}^2+\mathcal O(1).
\]
Row-wise lower isometry gives
\[
\mathcal E_t
\ge
\frac{t\mu_{\min}}8
\left\|
\widehat{\boldsymbol\alpha}
-\boldsymbol\alpha_\star
\right\|_\infty^2.
\]
Choosing $\theta$ sufficiently small absorbs the estimator-dependent
term, giving
\[
\left\|
\widehat{\boldsymbol\alpha}
-\boldsymbol\alpha_\star
\right\|_\infty^2
\lesssim
\epsilon_{\max}^2+\mathcal O(t^{-1}).
\]
Hence, $\epsilon_{\max}=O(t^{-1/2})$ yields the $t^{-1/2}$ rate. We state the formal theorem as:

\iffalse
First, martingale offset complexity retains the negative quadratic term in the basic inequality and yields
\[
\mathcal E_t\le c_1\theta t \|\hat{\boldsymbol\alpha}-\boldsymbol\alpha_\star\|_\infty^2+c_2t\epsilon_{\max}^2+\mathcal O(1).
\]
Second, row-wise lower isometry gives $\mathcal E_t\ge (t\underline\mu/8)\|\widehat{\boldsymbol\alpha}-\boldsymbol\alpha_\star\|_\infty^2$. Choosing $\theta$ small enough absorbs the estimator-dependent term, so
$\|\widehat{\boldsymbol\alpha}-\boldsymbol\alpha_\star\|_\infty^2\lesssim\epsilon_{\max}^2+\mathcal O(t^{-1})$. Thus a grid with $\epsilon_{\max}=O(t^{-1/2})$ gives $\|\widehat{\boldsymbol\alpha}-\boldsymbol\alpha_\star\|_\infty=\mathcal O(t^{-1/2})$.
\fi
Under \Cref{ass:stable_A}, define
\(
\epsilon_{\max}
:=
\max_{1\le i\le n}\epsilon_i,
\) \(
\mu_{\min}
:=
\min_{1\le i\le n}\mu_{t,i},
\) and $\Xi_t:=n\log(9n/\delta)+\log\det(\Gamma_t\Gamma_k^{-1})$. 
Fix $\delta\in(0,1/2)$ and choose
\(
0<\theta
\le
\min\left\{
\frac12,\,
\frac{
\delta\mu_{\min}
}{
576\sigma^2 n S_1^2
\operatorname{tr}(\Gamma_t)
}
\right\}.
\)
Suppose that the global separation condition holds:
\(
2\max_{1\le i\le n}
\Delta_t^{(i)}
\left(
\frac{\delta}{3n}
\right)
<
\min_{1\le i\le n}
\inf_{\substack{
\alpha\in\mathcal A_{\epsilon,i}\\
|\alpha-\alpha_{i,\star}|>\frac{\sigma\sqrt{\kappa_{i,\star}}}{2K_{i}(2+\|A_\star\|_\mathrm{op})}
}}
\left\{
R_t^{(i)}(\alpha)
-
R_t^{(i)}(\alpha_{\epsilon_i}^{\star})
\right\}.
\)
If
%\(
%t
%\ge
%t_{\mathrm{LI}}
%\left(
%\frac{\delta}{3}
%\right),
%\label{eq:LI_sample_size_fast_rate}
%\)
$t \gtrsim \left(n + \log\frac{n}{\delta} + \frac{1}{\min_i\underline{\alpha}_i^2} \log\frac{\sum_{i=1}^nM_i}{\delta} \right)$
and that, for some integer $k$,
\(
\frac{t}{k}
\ge
c\Xi_t.
\)
Then, with probability at least $1-\delta$,
\begin{align}
\left\|
\widehat{\boldsymbol{\alpha}}
-
\boldsymbol{\alpha}_\star
\right\|_\infty^2
\le{}&
\frac{
288\sigma^2 n S_1^2
\operatorname{tr}(\Gamma_t)
}{
\delta\mu_{\min}
}
\epsilon_{\max}^2
\nonumber\\
&+
\frac{
256\sigma^2
}{
3t\mu_{\min}\theta
}
\Bigg[
\left(
\sum_{i=1}^n
\log\frac{9M_i n}{\delta}
+
\log\frac{9}{\delta}
\right)
%\nonumber\\
%&\hspace{1.9cm}
+
\frac{
9C^2 n
\operatorname{tr}(\Gamma_t)
}{
\delta\lambda_{\min}(\Gamma_k)
}\Xi_t
\Bigg].
\end{align}
Consequently, if
\(
\epsilon_{\max}
=
\mathcal{O}\left(t^{-1/2}\right),
\)
then
\(
\left\|
\widehat{\boldsymbol{\alpha}}
-
\boldsymbol{\alpha}_\star
\right\|_\infty
=
\mathcal{O}\left(t^{-1/2}\right).
\)

\iffalse
\begin{theorem}[Fast rate for FO-GS]
Assume the Gaussian finite-past model, stability, and a global-separation condition that localizes
$|\widehat\alpha_i-\alpha_{i,\star}|\le\sqrt{\mu_{i,\mathrm{lb}}}/(2K_i)$, where
\[
\mu_{i,\mathrm{lb}}:=\frac{\sigma^2\kappa_{i,\star}}{2C_{\mathrm{der}}},
\qquad \underline\mu:=\min_i\mu_{i,\mathrm{lb}}>0.
\]
Let $M=\max_iM_i$, $\alpha_0=\min_i\underline\alpha_i$, and
$\Xi_t:=n\log(9n/\delta)+\log\det(\Gamma_t\Gamma_k^{-1})$. Suppose
\[
t\ge t_{\rm sep}(\delta/3)\vee t_{\rm LI}(\delta/3),
\qquad t/k\ge c\Xi_t,
\]
and choose
$0<\theta\le\min\{1/2,\delta\underline\mu/[576\sigma^2nS_1^2\operatorname{tr}(\Gamma_t)]\}$.
Then, with probability at least $1-\delta$,
\[
e_t^2\le C\!\left[
\frac{nS_1^2\operatorname{tr}(\Gamma_t)}{\delta\underline\mu}\epsilon_{\max}^2+
\frac{1}{t\underline\mu\theta}\!\left\{
\sigma^2\!\left(\sum_i\log\frac{9M_in}{\delta}+\log\frac9\delta\right)+
\frac{\sigma^2n\operatorname{tr}(\Gamma_t)}{\delta\lambda_{\min}(\Gamma_k)}\Xi_t
\right\}\right].
\]
Let
$\alpha_{\min}:=\min_i\alpha_{i,\star}$ and
$\kappa_{\min}:=\min_i\kappa_{i,\star}$. The two concentration
conditions above give
\[
t_{\rm LI}(\delta/3)=O\!\left(
\frac{C_{\rm der}^2}{\kappa_{\min}^2}
\left(n+\log\frac{n}{\delta}\right)
+
\frac{1}{\alpha_{\min}^2}
\log\frac{M_{\rm loc}}{\delta}
\right),
\]
where $M_{\rm loc}$ is the total number of local grid points. Thus the
new lower-isometry step introduces only an $\alpha_{\min}^{-2}$
requirement; the separate global-localization condition remains the
one already used in the paper.
If $\epsilon_{\max}=O(t^{-1/2})$, $\lambda_{\min}(\Gamma_k)=\Omega(1)$, and the grid/Gramian complexities are polylogarithmic, then
$e_t=\widetilde O(t^{-1/2})$.
\end{theorem}
\fi
Substituting this result into Theorem 2 gives
\[
\|\widehat A-A_\star\|_{\rm op}
\le C\sqrt{\frac{\Xi_t}{t\lambda_{\min}(\Gamma_k)}}
+CS_1 \left\|\widehat{\boldsymbol{\alpha}}-\boldsymbol{\alpha}_\star
\right\|_\infty \sqrt{\frac{n\widetilde C_G^2}{\delta\lambda_{\min}(\Gamma_{\lfloor k/2\rfloor})}}
=\mathcal{O}(t^{-1/2}).
\]
Thus both $\boldsymbol\alpha_\star$ and $A_\star$ achieve $t^{-1/2}$ rate. The improved rate is derived by combining the following two lemmas: controlling in-sample error via Martingale offset complexity and lower isometry.

\begin{lemma}
If $t/k\ge c\Xi_t$, then with probability at least $1-\delta$, for every $\tau\in(0,1]$ and $\rho>0$,
\[
\begin{aligned}
\mathcal E_t\le{}&(\tau+\rho)S_1^2\left\|
\widehat{\boldsymbol{\alpha}}-\boldsymbol{\alpha}_\star
\right\|_\infty^2\operatorname{tr}(X_tX_t^\top)
+3S_1^2\epsilon_{\max}^2\operatorname{tr}(X_tX_t^\top)\\
&+\frac{4(1+\rho^{-1})C^2\operatorname{tr}(X_tX_t^\top)}{t\lambda_{\min}(\Gamma_k)}\Xi_t
+\frac{8\sigma^2}{\tau}\sum_i\log\frac{3M_in}{\delta}
+8\sigma^2\log\frac3\delta .
\end{aligned}
\]
The coefficient $\tau+\rho$ is tunable and is absorbed by lower isometry.
\end{lemma}




\begin{lemma}
\label{lem:LI_rebuttal}
Suppose that the global separation condition holds. If
$t \gtrsim \left(n + \log\frac{n}{\delta} + \frac{1}{\min_i\underline{\alpha}_i^2} \log\frac{\sum_{i=1}^nM_i}{\delta} \right),$ then with probability at least $1-\delta$, simultaneously for all $i\in[n]$,
\[
\mathcal Q_{t,i}
\left(
\widehat\alpha_i,
\widehat a_i-a_{i,\star}
\right)
\ge
\frac{t\mu_{t,i}}{8}
|\widehat\alpha_i-\alpha_{i,\star}|^2.
\]
\end{lemma}

\iffalse
Thank you for raising this important point. We agree that our current $t^{-1/4}$ rate should not be interpreted as a fundamental lower bound, and we do not currently have a minimax lower bound showing that this rate is unavoidable. The$ t^{-1/4}$ rate arises from the proof technique used in the present analysis. Our proof first establishes a uniform deviation bound for the profiled squared loss by Lemma 1, $\max_{\alpha \in \mathcal{A}_{\epsilon,i}}\; \bigl|F_t^{(i)}(\alpha)-R_t^{(i)}(\alpha)\bigr| = O(t^{-1/2})$, and then combine this with the local quadratic-growth property of the population risk by lemma 2, $R_t^{(i)}(\alpha)-R_t^{(i)}(\alpha_{\star,i}) \gtrsim |\alpha - \alpha_{\star,i}|^2 $, which yields our current $ t^{-1/4} $ rate.

Determining the minimax rate, or developing a localized analysis that potentially achieves $t^{-1/2}$, is an important direction for future work. 
\fi

\textcolor{red}{Question 3: Is the $\alpha^{-8}$ requirement on $t$ tight? Since the method targets the small- $\alpha$ regime, please either tighten it or explain why such a strong dependence is necessary.}

Thank you for pointing this out. We agree that the previously stated $\alpha^{-8}$ requirement was not tight; it was an artifact of the global uniform convergence argument. In the revised theorem, we use a localization and lower-isometry argument, which yields the sufficient condition
\(
t
\gtrsim
n+\log\frac{n}{\delta}
+
\frac{1}{\min_i\underline{\alpha}_i^{2}}
\log\frac{\sum_{i=1}^{n}M_i}{\delta}.
\)
Thus, the $\alpha$ dependence is improved from $\alpha^{-8}$ to $\alpha^{-2}$.

The revised theorem still requires the global separation condition to distinguish the true fractional order from grid points outside its local neighborhood. This guarantees that $\hat{\alpha}_i$ lies in the region where the risk has sufficient curvature, enabling the fast-rate analysis.


\iffalse
Thank you for pointing this out. We agree that the $\alpha^{-8}$ dependence in the current theorem is not tight. It results from a coarse simplification of our concentration bound. The empirical process analysis in lemma 1 shows
$\Delta_t(\delta) = \mathcal{O} \Bigl(n^\frac{3}{2} \Bigl[\underline{\alpha}^{-2}\sqrt{\frac{n + \log(M/\delta)}{t}} + \underline{\alpha}^{-4} \frac{n + \log(M/\delta)}{t} \Bigr]  \Bigr)$. The two powers of $\alpha$ arise from the covariance sums associated with the fractional kernel. In particular, $\sum_{j \ge 1} j^{-(1+\alpha_i)} = O(\alpha_i^{-1})$, and $\sum_{j \ge 1} (1+ \log j) j^{-(1+\alpha_i)} = O(\alpha_i^{-2}) $, which lead to $ O(\alpha_i^{-4})$ constants in the quadratic-form concentration inequalities as $\alpha_i$ goes to 0. Consequently, their square-root contribution is  $ O(\alpha_i^{-2})$, whereas the linear tail contribution is  $ O(\alpha_i^{-4})$. 

In current version, for simplicity we upper-bounded both terms by $O \Bigl(n^\frac{1}{2} \underline{\alpha}_i^{-4}\sqrt{\frac{n + \log(M_i /\delta_i)}{t}} \Bigr)$, which produces the stated $\alpha^{-8}$ sample-size requirement when required to be smaller than a constant localization margin. This simplification is unnecessarily conservative. Retaining the original two-term bound, both conditions require only $t \gtrsim \alpha_i^{-4} $. We will therefore revise Lemma 1 and Theorem 1 to improve the sample requirement from  $ \alpha_i^{-8} $ to $ \alpha_i^{-4} $.   
\fi


\textcolor{red}{Question 4: Please add an integer-order OLS baseline and an ARFIMA baseline on the EEG data, to show whether the fractional model is actually needed. A log-log error-vs- plot over a wider horizon range would also let readers read off the empirical rate. }

The experiment is running.

\subsection{Reviewer gZM2}

\textcolor{red}{The symbol $\delta$  in Theorem 1 is never defined, nor does it make an appearance in Appendix E. There is a mention of  being fixed to a value in , but its actual meaning is never explained.
}

Thank you for pointing this out. We agree that the meaning of $\delta$ was not stated explicitly. In Theorem 1, $\delta \in (0, 1/2)$ is the failure probability of the finite-sample guarantee. For any prescribed $\delta$, the theorem guarantees that the stated estimation error bound holds with probability at least $1-\delta$ over the randomness of the observed trajectory.   

\textcolor{red}{The error bound for $|\hat{\alpha} - \alpha_\star|_\infty$ is inversely proportional to the measurement noise $\sigma$ , which is counter-intuitive.
As we discuss error bounds, it is worth pointing out that Theorem 2 sets (the order of which is omitted in the manuscript) to be independent of . In Simchowitz et al. (2018), it is explained that this is due to noise scaling, but this detail should not be omitted in your paper.
}

Thank you for pointing this out. We agree that the displayed dependence on $\sigma$ in Theorem 1 is misleading. The apparent $1/\sigma$ factor results from suppressing the $\sigma$ dependence in the $\mathcal{O} $ notation used for the uniform deviation bound $\Delta_t^{(i)}$. We thank the reviewer for catching this notational omission. 
Specifically, writing $\eta_s = \sigma \zeta_s$, where $\zeta_s \sim N(0, I)$, linearity of the FOLTI dynamics implies $x_s = \sigma \tilde{x}_s$, where $\tilde{x}_s$ is the is the corresponding trajectory with unit-variance process noise. Consequently, the empirical (Eq.(10)) and population risk (Eq.(11)) both scale as $\sigma^2$. Hence the factor $\sigma^2$ was absorbed into the $\mathcal{O} $ notation in the current manuscript. Likewise, the Lipschitz constant satisfies $L_{t,i} = \mathcal{O}(\sigma^2)$. Substituting these quantities into $|\hat{\alpha}_i-\alpha_{\star,i}|\le\sqrt{\frac{36\Delta_t^{(i)}(\delta/n)+18L_{i}\epsilon_i}{\sigma^2\kappa_{i,\star}}}$ shows that the $\sigma^2$ factors cancel.   

Therefore, the theorem does not predict that increasing the process-noise level improves estimation. The bound is invariant to a global rescaling of the process noise. We will revise Lemma 1 to make the $\sigma^2$ dependence explicit and remove the $1/\sigma$ dependence from the statement of Theorem 1.   

The fast rate bound is also independent of $\sigma$. Although the bound is written in terms of $\sigma^2/\mu_{\min}$, Lemma 12 gives $(\mu_{\min}=\Omega(\sigma^2))$, so the noise dependence cancels and the resulting rate is independent of $\sigma$.


\textcolor{red}{After L480 (Appendix B.1), you start making use of $y$  as a signal with the same sample-count as $x$, yet you never define it. This invalidates the subsequent proof steps.
Since we're here, right before this (L474) you restrict $\alpha_i$ to the open ball in $\mathbb{R}^n$ . Why can you make this assumption, and why do you use an open set?}

Thank you for catching this notational omission. We agree that $y_s^{(i)}$ should have been defined before L480. $y_s^{(i)}$ is a relabeling of  $\Delta^{\alpha_i} x_{s+1}^{(i)} $. With this definition, the expansion following L480 is simply the standard expansion of the centered squared loss, and the following argument remains unchanged.  

Thank you for pointing this out. We agree that the unit-ball restriction at L474 is not justified as currently written. We have now added a lemma showing that OLS estimators can be bounded by $R$ with high probability.
With probability at least $1-\delta$, the following holds
$\|\hat{a}_i(\alpha)\|_2 =\|(\Delta^{\alpha}X_t^{(i)})X_t^\top( X_tX_t^\top)^{-1} \|_2 \le \frac{8}{p} \sqrt{\frac{2\sigma^2n(t+1)\lambda_{\max}(\Gamma_{t+1})}{\delta k\lfloor t/k\rfloor\,\lambda_{\min}(\Gamma_{\mathrm{sb}}) }},$
for any $\alpha \in (0,1)$, and for any $k$ such that
$
\frac{t}{k}
\ge
c\!\left(
n\log(n/\delta)
+
\log\det(\Gamma_t\Gamma_k^{-1})
\right)
$.
Since $\lambda_{\max}(\Gamma_{t+1}) \le \tilde{C}_G^2 \zeta(2) $, the $R$ will not depend on $t$. Since FO-GS searches over a finite grid, applying this lemma to all grid candidates and taking a union bound gives $\hat{a}_i (\alpha) \in \mathbb{B}_R := \{a_i \in \mathbb{R}^{1 \times n} : \|a_i\|_2 < 1  \}$ for all candidates. 

We also agree that using an open ball is unnecessary and technically inappropriate here. We will replace it with the closed ball which ensures that the minimum is attained for the continuous quadratic loss. We thank the reviewer for identifying both issues. 

\textcolor{red}{Furthermore, confidence intervals should also be reported for the real-dataset results (e.g., via sample-error variance). }

Running experiments.

\textcolor{red}{L24-L25: You mention that classical Markovian models lack a mechanism to encode persistent historical influence and long-range correlations. However, Gu et al. (2020) achieve just that through a prescribed state-transition matrix that maximizes encoded history without resorting to fractional-order formulations. This is not to say that fractional-order systems have no use case, but the added complexity should be better motivated.}

Thank you for this important clarification. We agree that our statement at L24–L25 was too broad. Markovian state-space models can indeed represent long historical information when the state is appropriately augmented or specifically designed for memory. We will revise the introduction to avoid implying that Markovian models are fundamentally incapable of representing long-range dependence. Our motivation for fractional-order dynamics is more specific. We consider systems in which the observed physical state itself follows a nonlocal evolution law, rather than introducing an auxiliary latent state whose purpose is to summarize the past. This differs from HiPPO in both purpose and parameterization. HiPPO constructs a memory representation by projecting past inputs onto a prescribed polynomial basis, its state is explicitly designed to compress cumulative history. But in a fractional-order model the memory kernel is part of the unknown system dynamics, and the fractional order $\alpha$ controls the rate at which historical states influence the present. Thus, our goal is not to claim that fractional models are the only way to represent long memory, but to develop statistical identification guarantees when the data are generated by this particular class of non-Markovian dynamics.   

\textcolor{red}{Figure 1 uses an autocorrelation heatmap to motivate the long-range dependence of the example signal. However, the correlation energy is quite spread out, potentially suggesting that the temporal dependencies with older samples might be redundant with respect to. more recent values. The Partial Autocorrelation could easily get rid of this ambiguity.}

Thank you for this helpful suggestion. We would like to clarify, however, that Figure 1 is intended as a motivational illustration of long-range temporal correlation, rather than as an empirical identification argument for fractional-order dynamics. Long-range dependence is commonly reflected in a slowly decaying, typically power-law, autocorrelation structure, which is precisely the qualitative behavior illustrated in Figure 1. Our theoretical model is motivated directly by the Grünwald–Letnikov dynamics, where the past enters explicitly through coefficients whose magnitudes decay polynomially with the lag.  

\textcolor{red}{L58: you mention mild assumptions, but this is too ambiguous. Mild assumptions of what, exactly? Fractional-order regularity? System stability? Signal norm bounds?}

Thank you for pointing this out. We agree that “under mild assumptions” is vague. As detailed in our rebuttal to Reviewer VqoX, Question 1, we have now proved the former Assumption 2. Consequently, the revised main result requires only the fractional-system stability condition (Assumption 1). We will therefore replace “under mild assumptions” with “under the fractional system stability condition”.

\textcolor{red}{L78: Do [20,21,26] express this opinion, or are these examples of fractional-order SysID methods? Make this explicit in the text.}

Thank you for pointing this out. We agree that the current wording is ambiguous. References [20,21,26] are general references on fractional calculus and fractional-order systems, rather than examples of fractional-order system-identification methods. 

\textcolor{red}{L96: Missing domain for $s$.}

Thank you for catching this omission. The time index should be explicitly defined as $s = 0, 1, ..., t-1$.

\textcolor{red}{L120: even if $M_i$ is trivially $\frac{\bar{\alpha_i}-\underline{\alpha}_i}{\epsilon_i}$, it should still be defined.}

Thank you. Define $M_i = \frac{\bar{\alpha_i}-\underline{\alpha}_i}{\epsilon_i} $.

\textcolor{red}{Equation 7: Is it not $\arg\min$?}

Yes, thanks for catching this typo. Equation (7) should use $\arg\min$.


\textcolor{red}{Equation 8: If you're optimizing $\alpha \in \mathcal{A}_{\epsilon,i}$, you should use it without subscripts in the loss function. Otherwise, use $\alpha_{i,k} \in \mathcal{A}_{\epsilon,i}$}. 

Thank you for catching this notation inconsistency. We will replace $\alpha_{i,k}$ by $\alpha$ in Eq.(8) for consistency.

\textcolor{red}{Equation 9: For consistency, use $X_{t-1} = [x_0, \ldots, x_{t-1}].$ }

Thank you for pointing this out. We agree that the current notation can be confusing. We will denote it consistently as  $X_{t-1} = [x_0, \ldots, x_{t-1}].$ and revise Eq. (9) and the subsequent proof accordingly. This is purely a notation change and does not affect the estimator or theoretical results.

\textcolor{red}{L134: Missing domain for $z$ (real or complex?)}

Thank you for pointing this out. Here z is complex-valued with $|z| \le 1$.

\textcolor{red}{L279: It is not a good idea to analyze results relegated to the appendix in the main text. Analysis of the latter should be self-contained.}

Thank you for this suggestion. We agree that the main text should be self-contained. The statement at L279 (“Training errors are similar across methods”) refers to Figure 4 in the appendix and is not necessary for interpreting the main result in Figure 3. We will therefore remove this statement from the main text and discuss the training-error comparison together with Figure 4 in the appendix. The main text will focus on the test NMSE reported in Figure 3.

\textcolor{red}{The hardware specs should be reported in the main text, as the checklist will not be part of the final manuscript.}

Thank you for pointing this out. We will add to the experimental setup that all experiments were conducted on a workstation with an NVIDIA GeForce RTX 5080 GPU and an AMD Ryzen 7 9800X3D CPU.

\textcolor{red}{The real-world dataset is an external asset, and its license should be reported (or it should be noted in the main text that there is no license attached).}

Thank you for pointing this out. We will add the dataset source, version, and license to the main text.

\textcolor{red}{Layout:
Section 5 would work better if carefully combined with Section 4.2. In its current format, it forces the reader to go back and forth between pages.
Arrange appendices according to the order of mention in the main text.}

Thank you for the helpful suggestions. We will merge Section 5 with Section 4.2 so that the corresponding results and discussion can be read continuously without requiring the reader to navigate back and forth. We will also reorder the appendices to follow their first occurrence in the main text, making the paper easier to navigate.

\textcolor{red}{In L41-L43, you use the terms heterogeneous and commensurate to refer to multiple and single fractional orders, respectively. Wouldn't heterogeneous/homogeneous sound more consistent?
L67: ...branch of fractional-order system identification...
L71: not expend; either expand or extend.
L73: ...the diagonal structure...
L77-L78: While the system identification for ordinary LTI systems is a relatively well-understood field...
L82: ...conditioned on these estimates...
L84-L85: Either Chatterjee and Pequito study..., or The work in Chatterjee and Pequito studies...; same for establishes.
L93: ...difference of the form
L116: ...we define
L132: ...for simplicity of proof.
L150: This assumption...
L153: Put We are now ready... into a new paragraph.
L217: To ensure all 
...
L266: We studied how the number of grid points 
...
L270: ...roughly ten grid points and in estimating $A$ with roughly five grid points.
Figure 2: Number of grid points instead of number of grids.
L293: Future work should focus on reducing the grid-search cost...}

Thank you for these careful language and presentation suggestions. We agree with the proposed terminology, grammatical corrections, paragraphing, and figure-label changes, and will revise the manuscript accordingly. We will also improve the wording around the grid-search discussion and clarify the future-work statement on reducing computational cost.

\textcolor{red}{Question 1: Did you inspect the learned fractional orders for the real dataset? What conclusions can be drawn from these?}

We inspected the learned fractional orders on the EEG dataset and found clear evidence of non-integer, channel-dependent memory. For \textit{FO-GS}, the median window-averaged order is (0.855); (74.6\%) of windows have a cross-channel order range greater than (0.5), and (72.8\%) contain at least one channel with $\alpha \le 0.1$. Because smaller $\alpha$ corresponds to a more slowly decaying Grünwald--Letnikov memory kernel, these results suggest substantial heterogeneity in long-term memory across EEG channels.

The baseline comparison supports this conclusion. Although \textit{FO-BS} has a similar median order of (0.857), \textit{FO-GS} produces a larger cross-channel range in (72.3\%) of paired windows. Moreover, the proportions of windows with range greater than (0.5) and with at least one $\alpha \le 0.1$ are (74.6\%) and (72.8\%) for \textit{FO-GS}, compared with (57.2\%) and (59.4\%) for \textit{FO-BS}. In contrast, \textit{FO-WT} concentrates near the integer-order boundary: its median mean order is (0.949), and (94.0\%) of windows have mean order above (0.9). We will add these statistics to show that \textit{FO-GS} captures richer heterogeneous memory structure, in addition to improving prediction.

Yes. We inspected the learned fractional orders on the EEG dataset, and they reveal substantial non-integer and channel-dependent memory structure. \textit{FO-GS} has a median window-averaged order of 0.855, 74.6\% of windows have an order range larger than 0.5, and 72.8\% contain at least one channel with $\alpha \le 0.1$. Since smaller $\alpha$ induces a slower decaying Grünwald–Letnikov memory kernel, this suggests that some EEG channels exhibit substantially stronger long-term memory than others.

The comparison with the baselines is also informative. \textit{FO-BS} obtains a very similar median window-averaged order (0.857), but \textit{FO-GS} identifies stronger cross-channel heterogeneity: \textit{FO-GS} has a larger order range in 72.3\% of paired windows, and the fraction of windows with range larger than $0.5$ is 74.6\% for \textit{FO-GS} versus 57.2\% for \textit{FO-BS}. Likewise, the fraction containing a strongly long-memory channel $\alpha \le 0.1$ is 72.8\% versus 59.4\%.

In contrast, \textit{FO-WT} estimates concentrate near the upper boundary: its median mean order is 0.949, and 94.0\% of windows have mean order above 0.9. Thus, \textit{FO-WT} largely produces nearly homogeneous, near-integer orders, whereas \textit{FO-GS} reveals substantially richer channel-dependent memory. We will add these fractional-order statistics to the real-data analysis to clarify that \textit{FO-GS} provides not only predictive gains, but also an interpretable characterization of heterogeneous long-term memory in the EEG signals.

\textcolor{red}{Question 2: Why does the synthetic $\alpha$
 grid stop at 0.5? What happens (in practice) as you allow the method to explore fractional orders $\alpha\to 1$?}

Thank you for raising this point. The original synthetic range $\alpha \le 0.5$ was chosen to emphasize the long-memory regime, and it is not an algorithmic restriction of \textit{FO-GS}. To address the reviewer’s concern, we added new experiments with $\alpha \in [0.5, 0.99]$, varying the noise level, time horizon, and grid size. The following tables show that \textit{FO-GS} remains consistently more accurate than baselines throughout this high $\alpha$ regime.

For \(\alpha\)-MSE, FO-BS achieves \(0.02778 \pm 0.00298\) and FO-WT achieves \(0.01294 \pm 0.00201\). For \(A\)-MSE, FO-BS achieves \(0.02798 \pm 0.00412\) and FO-WT achieves \(0.00680 \pm 0.00174\).

\begin{table}[t]
\centering
\caption{MSE of \(\alpha\) under different noise levels $\sigma$.}
\label{tab:alpha_mse}
\small
\begin{tabular}{cccc}
\toprule
\(\sigma\) & \textit{FO-GS} & \textit{FO-BS} & \textit{FO-WT} \\
\midrule
0.05 & \(0.00440 \pm 0.00182\) & \(0.05135 \pm 0.00706\) & \(0.03237 \pm 0.00475\) \\
0.10 & \(0.00591 \pm 0.00253\) & \(0.07113 \pm 0.00660\) & \(0.03361 \pm 0.00508\) \\
0.20 & \(0.00975 \pm 0.00237\) & \(0.08218 \pm 0.00532\) & \(0.03541 \pm 0.00480\) \\
0.30 & \(0.01224 \pm 0.00392\) & \(0.08286 \pm 0.00523\) & \(0.03859 \pm 0.00531\) \\
0.40 & \(0.01154 \pm 0.00274\) & \(0.08474 \pm 0.00505\) & \(0.04405 \pm 0.00516\) \\
0.50 & \(0.01361 \pm 0.00376\) & \(0.08527 \pm 0.00490\) & \(0.04401 \pm 0.00546\) \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{MSE of \(A\) under different noise levels $\sigma$.}
\label{tab:A_mse}
\small
\begin{tabular}{cccc}
\toprule
\(\sigma\) & \textit{FO-GS} & \textit{FO-BS} & \textit{FO-WT} \\
\midrule
0.05 & \(0.001366 \pm 0.000488\) & \(0.03604 \pm 0.00540\) & \(0.00730 \pm 0.00154\) \\
0.10 & \(0.002341 \pm 0.000810\) & \(0.04605 \pm 0.00580\) & \(0.00762 \pm 0.00215\) \\
0.20 & \(0.003171 \pm 0.000965\) & \(0.05524 \pm 0.00702\) & \(0.00689 \pm 0.00174\) \\
0.30 & \(0.005507 \pm 0.001755\) & \(0.05378 \pm 0.00623\) & \(0.00680 \pm 0.00145\) \\
0.40 & \(0.004532 \pm 0.000997\) & \(0.05875 \pm 0.00672\) & \(0.00817 \pm 0.00143\) \\
0.50 & \(0.005590 \pm 0.001933\) & \(0.05969 \pm 0.00871\) & \(0.00962 \pm 0.00191\) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[t]
\centering
\caption{MSE of $\alpha$ under different time horizons \(T\).}
\label{tab:alpha_mse_T}
\small
\begin{tabular}{cccc}
\toprule
\(T\) & \textit{FO-GS} & \textit{FO-BS} & \textit{FO-WT} \\
\midrule
100 & \(0.00820 \pm 0.00267\) & \(0.03878 \pm 0.00494\) & \(0.02078 \pm 0.00455\) \\
200 & \(0.00470 \pm 0.00156\) & \(0.03982 \pm 0.00489\) & \(0.02528 \pm 0.00536\) \\
300 & \(0.00266 \pm 0.00067\) & \(0.04075 \pm 0.00454\) & \(0.02776 \pm 0.00548\) \\
400 & \(0.00168 \pm 0.00042\) & \(0.04301 \pm 0.00467\) & \(0.02618 \pm 0.00560\) \\
500 & \(0.00223 \pm 0.00060\) & \(0.04391 \pm 0.00474\) & \(0.02762 \pm 0.00551\) \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{MSE of $A$ under different time horizons \(T\).}
\label{tab:A_mse_T}
\small
\begin{tabular}{cccc}
\toprule
\(T\) & \textit{FO-GS} & \textit{FO-BS} & \textit{FO-WT} \\
\midrule
100 & \(0.005833 \pm 0.001932\) & \(0.03434 \pm 0.00443\) & \(0.01004 \pm 0.00314\) \\
200 & \(0.002101 \pm 0.000849\) & \(0.02335 \pm 0.00319\) & \(0.004270 \pm 0.001169\) \\
300 & \(0.001023 \pm 0.000271\) & \(0.02404 \pm 0.00281\) & \(0.004243 \pm 0.001548\) \\
400 & \(0.000637 \pm 0.000210\) & \(0.02373 \pm 0.00311\) & \(0.003316 \pm 0.001009\) \\
500 & \(0.000921 \pm 0.000335\) & \(0.02289 \pm 0.00258\) & \(0.003606 \pm 0.000925\) \\
\bottomrule
\end{tabular}
\end{table}
\iffalse
\begin{table}[t] 
\centering 
\caption{\textit{FO-GS} performance under different grid sizes $M$.} 
\label{tab:memory_length_mse} 
\small 
\begin{tabular}{ccc} 
\toprule \(M\) & FO-GS \(\alpha\)-MSE & FO-GS \(A\)-MSE \\ \midrule 2 & \(0.03021 \pm 0.00448\) & \(0.01414 \pm 0.00451\) \\ 3 & \(0.01338 \pm 0.00330\) & \(0.00829 \pm 0.00253\) \\ 4 & \(0.01086 \pm 0.00280\) & \(0.00786 \pm 0.00239\) \\ 5 & \(0.00891 \pm 0.00275\) & \(0.00628 \pm 0.00224\)  \\ 10 & \(0.00856 \pm 0.00278\) & \(0.00642 \pm 0.00230\) \\ 15 & \(0.00812 \pm 0.00255\) & \(0.00605 \pm 0.00213\) \\ 20 & \(0.00839 \pm 0.00264\) & \(0.00626 \pm 0.00219\) \\ 25 & \(0.00837 \pm 0.00268\) & \(0.00630 \pm 0.00224\) \\ \bottomrule \end{tabular}
\end{table}
\fi
\begin{table}[t] 
\centering 
\caption{\textit{FO-GS} performance under different grid sizes $M$.} 
\label{tab:memory_length_mse} 
\small 
\begin{tabular}{ccc} 
\toprule \(M\) & \(\alpha\) MSE & \(A\) MSE \\ \midrule 2 & \(0.03021 \pm 0.00448\) & \(0.01414 \pm 0.00451\) \\  
4 & \(0.01086 \pm 0.00280\) & \(0.00786 \pm 0.00239\) \\ 
\textbf{5} & \(\boldsymbol{0.00891 \pm 0.00275}\) & \(\boldsymbol{0.00628 \pm 0.00224}\)  \\ 
10 & \(0.00856 \pm 0.00278\) & \(0.00642 \pm 0.00230\) \\ 
15 & \(0.00812 \pm 0.00255\) & \(0.00605 \pm 0.00213\) \\ 
\bottomrule \end{tabular}
\end{table}


 \clearpage
 \textcolor{red}{Question 3: Were the synthetic system dynamics purely real? What happens when complex-conjugate eigenvalues are introduced?}

Thank you for raising this point. The original synthetic experiments used \(A\) with real eigenvalues. This is an experimental choice rather than a restriction of \textit{FO-GS} or our theory. \textit{FO-GS} operates directly on the state-space regression and does not require an eigendecomposition or a real spectrum. 

Our theoretical results also do not assume that the eigenvalues of $A$ are real; they require the fractional stability condition in Assumption 1. Therefore, complex-conjugate modes are covered whenever this condition holds.

\[
\left\|
\left(
\sum_{s=0}^{T-1} b_s(\alpha)x_s^\top
\right)
\left(
\sum_{s=0}^{T-1} x_s x_s^\top
\right)^{-1/2}
\right\|_F
\asymp
\sqrt{T}\,\|\alpha-\alpha^\star\|.
\]

\subsection{Reviewer HCia}
\textcolor{red}{What guarantees that \(X_t X_t^\top\) is invertible and well-conditioned at finite t, especially for the EEG case (n=19 from about 105 correlated samples)?}

Thank you for raising this point. In the theoretical setting, invertibility is guaranteed at finite $t$ through the block martingale small-ball (BMSB) argument in Appendix C.1 Eq(67). We show that with high probability
$X_t X_t^\top \succeq \frac{p^2}{16}\,k\lfloor t/k\rfloor \Gamma_{\mathrm{sb}}$. Since $G_0 = I$ and $H_{\lfloor k/2\rfloor} \succeq I$, then $\Gamma_{\mathrm{sb}}=\sigma^2 H_{\lfloor k/2\rfloor} \succ 0$. Therefore, once the condition in Lemma 3 is satisfied, $\lambda_{\min}(X_tX_t^\top) >0 $ with high probability.

For the EEG experiments, we use ridge regularization with $\lambda = 10^{-8}$ for numerical robustness. We additionally checked the rank of $X_t$ in the first dataset: 200 of 206 windows (97.1\%) have full rank.

\textcolor{red}{How do the bound and the sample-size condition depend on the dimension n and on the smallest fractional order, and can you please test beyond $n = 2$ and in a small alpha (strong long memory case) setting?}

The dependence can be summarized separately for the two parameters $\alpha$ and $A$. For the fractional order $\alpha$, Theorem 1 shows that the required sample size grows approximately linearly with $n$ and as $\underline{\alpha}^{-4}$ (See the rebuttal to Reviewer VqoX's Question 2). The estimation error grows approximately linearly with $n$ and as $\underline{\alpha}^{-2}$.

For the system matrix $A$, the sample size condition inherits the $\underline{\alpha}^{-4}$ from estimating $\alpha$ and grows approximately linearly with $n$. The estimation error grows approximately $n^{3/2}\underline{\alpha}^{-2}$. 

\textcolor{red}{What is the actual cost of FO-GS in terms of (n, M, t) given the full history convolution, and how many grid points are really needed at the largest t? Theorem 1 seems to require M=O(sqrt(t)), which doesn't match the about ten grids suffice result you mentnioned at t = 100.}

Thank you for raising this question. Here, $M$ denotes the number of grid points per fractional-order coordinate, while the history length in the Grünwald--Letnikov convolution is $t$. Because *FO-GS* performs a row-wise search, it evaluates only $nM$ candidates, rather than the $M^n$ points of a Cartesian search.

**Computational cost.** The state Gram matrix $X_tX_t^\top$ and its inverse are computed once, at costs $O(n^2t)$ and $O(n^3)$, respectively. For each row and each grid point, directly computing the full-history fractional convolution costs $O(t^2)$, while computing the profiled OLS estimator and loss costs $O(nt+n^2)$. Therefore, the total serial complexity is
$
O\!\left(n^2t+n^3+nM(t^2+nt+n^2)\right).
$
In the typical regime $t\gtrsim n$, the full-history convolution dominates, giving $O(nMt^2)$. Grid candidates and rows are also independently parallelizable.

**Original $t^{-1/4}$ theorem.** The old Theorem 1 contains a statistical error of order $\mathcal{O}(t^{-1/4})$ and a grid-discretization error of order $O(\sqrt{\epsilon})$. Balancing them gives $\epsilon=O(t^{-1/2})$, and hence $M=O(\sqrt t)$ on a fixed bounded search interval. This is consistent with the grid size experiment: at $t=100$, $\sqrt{t}=10$, so the observation that roughly ten grid points suffice does not contradict the theorem. Our statement that about ten grid points suffice was specific to the experiment at $t=100$, rather than a claim that ten points suffice for arbitrarily large $t$. The largest experimental horizon is $t=500$; extrapolating the same scaling gives approximately $22$ grid points, while we use 20 points in the trajectory horizon experiments. The theorem provides a sufficient asymptotic scaling, rather than an exact minimum number of grid points.

**Revised $t^{-1/2}$ theorem.** In the new fast-rate theorem, the squared estimation error has the form
$
\|\widehat{\boldsymbol{\alpha}}-\boldsymbol{\alpha}_\star\|_\infty^2
\lesssim
\epsilon_{\max}^2+
\widetilde O\!\left(\frac{\sum_i\log M_i}{t}\right),
$
up to the stated system-dependent quantities. Choosing
$
\epsilon_{\max}=\mathcal{O}(t^{-1/2})
$
therefore preserves the $\widetilde O(t^{-1/2})$ statistical rate, again corresponding to $M=\mathcal{O}(\sqrt t)$ for a one-stage uniform grid.

\textcolor{red}{Are (alpha, A) jointly identifiable? In ARFIMA the long and short-memory parts are known to trade off in finite samples, and estimating alpha first and then fitting A by OLS is the two-step setup that tends to be biased.}


Yes, $(\alpha,A)$ are jointly identifiable under our excitation and separation conditions. The key distinction from a conventional two-step estimator is that \textit{FO-GS} does not estimate $\alpha$ independently and then treat it as fixed when estimating $A$.



For every candidate $\alpha$, it computes
\[\widehat{A}(\alpha)
=
\arg\min_A L_t(\alpha,A),
\]
and then selects $\widehat{\alpha}$ by minimizing the profiled loss
\[
L_t\bigl(\alpha,\widehat{A}(\alpha)\bigr).
\]
Equivalently,
\[
(\widehat{\alpha},\widehat{A})
=
\arg\min_{\alpha,A} L_t(\alpha,A),
\]
up to the discretization of the $\alpha$-grid. Thus, our method is a joint least-squares estimator implemented through profiling, rather than a plug-in two-step estimator that first estimates $\alpha$ and subsequently fits $A$ while keeping $\alpha$ fixed.

Intuitively, changing $A$ may partially compensate for an incorrect $\alpha$ through the most recent state, but it cannot reproduce the full history-dependent convolution induced by the fractional-difference operator. Under sufficient state excitation, these additional lagged terms distinguish different values of $\alpha$. The separation condition ensures that the population profiled risk has a unique minimizer at $\alpha_\star$, while the nonsingularity of the state covariance identifies $A_\star$ once $\alpha_\star$ is fixed. We agree that finite-sample tradeoffs may still increase the estimation error, especially for short trajectories or strong long-memory regimes; these effects are reflected in our finite-sample curvature and separation quantities.



Yes, $(\boldsymbol{\alpha},A)$ are jointly identifiable under the nonsingularity, curvature, and separation conditions used in our analysis. The key distinction from a conventional two-step estimator is that \textit{FO-GS} does not estimate $\boldsymbol{\alpha}$ independently and then treat it as fixed when estimating $A$.

Specifically, for each row $i$ and every candidate $\alpha_i$, \textit{FO-GS} computes
$
\hat a_i(\alpha_i)
\in
\arg\min_{a_i}
\mathcal{L}^{(i)}(\alpha_i,a_i),
$
and then selects
$
\hat\alpha_i
\in
\arg\min_{\alpha_i\in\mathcal A_{\epsilon,i}}
\mathcal{L}^{(i)}
\bigl(\alpha_i,\hat a_i(\alpha_i)\bigr).
$
Equivalently,
$
(\hat{\boldsymbol{\alpha}},\hat A)
\in
\arg\min_{\boldsymbol{\alpha}\in\mathcal A_\epsilon,\,A}
\mathcal{L}(\boldsymbol{\alpha},A).
$
Thus, our procedure is a joint least-squares estimator implemented through profiling, rather than a plug-in estimator that first estimates $\boldsymbol{\alpha}$ and subsequently fits $A$ while keeping $\boldsymbol{\alpha}$ fixed.

Changing $A$ may partially compensate for an incorrect $\alpha_i$, which is precisely why our analysis profiles out $a_i$. After profiling, the condition $\mu_{t,i}>0$ ensures that the history-dependent derivative signal induced by changing $\alpha_i$ cannot be fully represented by a linear function of the current state. This yields local identifiability of $\alpha_i$, while the global separation condition rules out competing minimizers outside the local neighborhood. Once $\boldsymbol{\alpha}_\star$ is identified, the nonsingularity of the state Gram matrix $X_tX_t^\top$ identifies $A_\star$ through OLS. We agree that finite-sample tradeoffs can still increase estimation error, especially for short trajectories or strong long-memory regimes. These effects are captured by the curvature and separation quantities in our finite sample bounds.

Our results establish recovery of $(\boldsymbol{\alpha}_\star,A_\star)$
under local curvature and global separation conditions in our
theory; we do not claim unconditional joint identifiability for every
fractional-order system.

\textit{FO-GS} is implemented in two stages. For each row $i$ and every candidate $\alpha_i$, \textit{FO-GS} computes
$
\hat a_i(\alpha_i)
\in
\arg\min_{a_i}
\mathcal{L}^{(i)}(\alpha_i,a_i),
$
and then selects
$
\hat\alpha_i
\in
\arg\min_{\alpha_i\in\mathcal A_{\epsilon,i}}
\mathcal{L}^{(i)}
\bigl(\alpha_i,\hat a_i(\alpha_i)\bigr).
$
Equivalently,
$
(\hat{\boldsymbol{\alpha}},\hat A)
\in
\arg\min_{\boldsymbol{\alpha}\in\mathcal A_\epsilon,\,A}
\mathcal{L}(\boldsymbol{\alpha},A).
$
Thus, $A$ is not estimated only after fixing a separately obtained
estimate of $\boldsymbol{\alpha}$. Instead, $a_i$ is optimized for every candidate $\alpha_i$, and the
$(\alpha_i,a_i)$ pair is selected through the profiled least-squares
loss.

The possible finite-sample tradeoff between $\alpha_i$ and $a_i$ is
therefore not ignored: profiling allows $a_i$ to provide its best
possible compensation for each candidate $\alpha_i$. Our positive
profiled curvature $\mu_{t,i}$ ensures local separation even after
optimizing over $a_i$, while the global separation condition rules out
competing profiled-risk minimizers outside this neighborhood.

\clearpage




